BundleFlow: Deep Menus for Combinatorial Auctions by Diffusion-Based Optimization

Differentiable economics -- the use of deep learning for auction design -- has driven progress in the automated design of multi-item auctions with additive or unit-demand valuations. However, little progress has been made for optimal combinatorial auctions (CAs), even for the single bidder case, because we need to overcome the challenge of the bundle space growing exponentially with the number of items. For example, when learning a menu of allocation-price choices for a bidder in a CA, each menu element needs to efficiently and flexibly specify a probability distribution on bundles. In this paper, we solve this problem in the single-bidder CA setting by generating a bundle distribution through an ordinary differential equation (ODE) applied to a tractable initial distribution, drawing inspiration from generative models, especially score-based diffusion models and continuous normalizing flow. Our method, BundleFlow, uses deep learning to find suitable ODE-based transforms of initial distributions, one transform for each menu element, so that the overall menu achieves high expected revenue. Our method achieves 1.11$-$2.23$\times$ higher revenue compared with automated mechanism design baselines on the single-bidder version of CATS, a standard CA testbed, and scales to problems with up to 150 items. Relative to a baseline that also learns allocations in menu elements, our method reduces the training iterations by 3.6$-$9.5$\times$ and cuts training time by about 80% in settings with 50 and 100 items.

==> backup.tex <==
\begin{theorem}[Locally-Extending Mutual Compatibility]\label{thm:2_bidder_comp} For the two-bidder case, $\vv$ = ($\vv_i$, $\vv_{\shortn i}$) is a grid point used in the transformation, then $\forall \vv'\in\mathcal{N}_{\frac{\epsilon}{2}}=\{\vv' | \|\vv'-\vv\|\le \epsilon / 2\}$ is compatible.
\end{theorem}
\begin{proof}
(I) We first consider a fixed grid point of bidder $\shortn i$'s value, to which a transformation procedure is applied. Here the menu $B_i$ of bidder $i$ is unchanged. Suppose that bidder $i$ selects the $k_i$-th element $(\bm\alpha_i^{(k_i)}, \beta_i^{(k_i)})$ in this menu when its type is $\vv_i$, and bidder $\shortn i$ selects the $k_{\shortn i}$-th in its menu $B_{\shortn i}(\vv_i)$ when bidder $i$ is of the type $\vv_i$. The bidders' menu selections $k_i$ and $k_{\shortn i}$ are compatible due to our transformation process. We now prove that the mutual compatibility of allocation holds for all values in $\mathcal{N}_{i,\frac{\epsilon}{2}}=\{\vv_i' | \|\vv_i'-\vv_i\|_\infty\le \epsilon / 2\}$.

(I.A) Case 1: Both bidders do not change their menu element selection in \neighbor. In this case, the only possibility of incompatibility comes from the change in the allocation of bidder $\shortn i$, $\bm\alpha_{\shortn i}^{(k_{\shortn i})}(\vv_i)$, due to the varying $\vv_i$ value (recall that $\bm\alpha_{\shortn i}^{(k_{\shortn i})}$ is generated by the allocation network that is conditioned on $\vv_i$). With the Lipschitz constant $L_a$ of our allocation network, this change can be bounded by:
\begin{align}
    \|\Delta \bm\alpha_{\shortn i}^{(k_{\shortn i})}\|_\infty \le L_a \|\Delta \vv_i\|_\infty \le \frac{\epsilon}{2}L_a.
\end{align}
Here our safety margin $s_f= \frac{\epsilon}{2}L_a $ comes into play. With $s_f$ in the incompatibility loss (Eq.~\ref{equ:f_loss}) and the transformation process (Eq.~\ref{equ:mip_feas_standard}), we have
\begin{align}
    \bm\alpha_i^{(k_i)}+\bm\alpha_{\shortn i}^{(k_{\shortn i})} \le 1 - s_f \le 1 - \Delta \bm\alpha_{\shortn i}^{(k_{\shortn i})}.
\end{align}
It follows that $\bm\alpha_i^{(k_i)}+\bm\alpha_{\shortn i}^{(k_{\shortn i})}+\Delta \bm\alpha_{\shortn i}^{(k_{\shortn i})}\le 1$, which means the joint allocation is always feasible in \neighbor.

(I.B) For the other cases, we need the condition that bidder $\shortn i$ does not change its selection in \neighbor. We first prove that if, at $\vv_i$, the utility of the best element in bidder $\shortn i$'s menu is at least $s_m=2(v_{\max}L_a + L_p)\epsilon$ higher than that of the second best element, then bidder $\shortn i$ does not change its selection in \neighbor. Here, $v_{\max}$ is the maximum possible value and $L_p$ is the Lipschitz constant of our payment network. 

Assume that bidder $\shortn i$ changes from $k_{\shortn i}$-th element to a second menu element $(\bm\alpha_{\shortn i}^{(k_{\shortn i}')}, \beta_{\shortn i}^{(k_{\shortn i}')})$ at $\vv_i'$. At $\vv_i$, we have
\begin{align}
    &\vv_{\shortn i}^\Tau \bm\alpha_{\shortn i}^{(k_{\shortn i})}(\vv_i) - \beta_{\shortn i}^{(k_{\shortn i})}(\vv_i) \nonumber\\
    \ge &\vv_{\shortn i}^\Tau \bm\alpha_{\shortn i}^{(k_{\shortn i}')}(\vv_i) - \beta_{\shortn i}^{(k_{\shortn i}')}(\vv_i) + s_m \\
    \ge &\vv_{\shortn i}^\Tau \bm\alpha_{\shortn i}^{(k_{\shortn i}')}(\vv_i) - \beta_{\shortn i}^{(k_{\shortn i}')}(\vv_i) + 2(v_{\max}L_a + L_p)\|\vv_i'-\vv_i\|_\infty.\label{equ:case22-1}\nonumber
\end{align}
Then, at $\vv_i'$, it follows that:
\begin{align}
    & \vv_{\shortn i}^\Tau \bm\alpha_{\shortn i}^{(k_{\shortn i})}(\vv_i') - \beta_{\shortn i}^{(k_{\shortn i})}(\vv_i') \\
    \ge & \vv_{\shortn i}^\Tau \bm\alpha_{\shortn i}^{(k_{\shortn i})}(\vv_i) - \beta_{\shortn i}^{(k_{\shortn i})}(\vv_i) - (v_{\max}L_a + L_p)\|\vv_i'-\vv_i\|_\infty\nonumber \\
    \ge & \vv_{\shortn i}^\Tau \bm\alpha_{\shortn i}^{(k_{\shortn i}')}(\vv_i) - \beta_{\shortn i}^{(k_{\shortn i}')}(\vv_i) + (v_{\max}L_a + L_p)\|\vv_i'-\vv_i\|_\infty\nonumber\\
    \ge & \vv_{\shortn i}^\Tau \bm\alpha_{\shortn i}^{(k_{\shortn i}')}(\vv_i') - \beta_{\shortn i}^{(k_{\shortn i}')}(\vv_i')\label{equ:case22-2},
\end{align}
which means that bidder $\shortn i$ would still select $k_{\shortn i}$ at $\vv_i'$. 

The question then becomes how to guarantee a safety margin of $s_m=2(v_{\max}L_a + L_p)\epsilon$. Our findings indicate that for the network-generated menus of most $\vv_i$, this criterion is already met. Therefore, in practice, after sampling and prior to transforming, we verify whether this condition is satisfied for each $\vv_i\in\mathcal{V}_i$. If it is not, we add a new grid point to reduce $\epsilon$ to $\epsilon/2$. This procedure can be repeated until the condition is met.
% , or until $\epsilon/2$ is sufficiently small. In such cases, we can freeze bidder $\shortn i$'s selection in \neighbor~without significantly impacting revenue. \twadd{+ A justification for not violating IC with this freezing.}

% \twadd{Check this} The agent can always choose to select the IR option if $k_{\shortn i}$ gives him less than $0$ in utility. We note, however, that the compatibility constraint is further relaxed whenever IR is selected since the allocation probability is $0$ under the IR option, therefore we can focus on the case that bidder $\shortn i$ would not change its selection in \neighbor~without loss of generality.

Now we can discuss the case where bidder $i$ changes its menu element selection in \neighbor. Suppose that bidder $i$ changes from $k_i$-th element to another menu element $(\bm\alpha_i^{(k_i')}, \beta_i^{(k_i')})$ at $\vv_i'$. If $\bm\alpha_i^{(k_i')}$ is incompatible with $\bm\alpha_{\shortn i}^{(k_{\shortn i})}$, our construction of bidder $i$'s menu transformation process (Eq.~\ref{eq:trans_infeas}) requires that, at $\vv_i$: (Here $s_t=\epsilon/2$)
\begin{align}
    &\vv_i^\Tau \bm\alpha_i^{(k_i)} - \beta_i^{(k_i)} \ge \vv_i^\Tau \bm\alpha_i^{(k_i')} - \beta_i^{(k_i')} + s_t\nonumber \\
    \Rightarrow\ \ & \left(\vv_i^{\Tau} \bm\alpha_i^{(k_i)} - \beta_i^{(k_i)}\right) - \left(\vv_i^{\Tau} \bm\alpha_i^{(k_i')} - \beta_i^{(k_i')}\right) \ge \|\vv_i'-\vv_i\|_1\label{equ:case32-1}
\end{align}


At $\vv_i'$, it follows that:
\begin{align}
    & \left(\vv_i^{'\Tau} \bm\alpha_i^{(k_i)} - \beta_i^{(k_i)}\right) - \left(\vv_i^{'\Tau} \bm\alpha_i^{(k_i')} - \beta_i^{(k_i')}\right) \nonumber\\
    = & \left[\vv_i^{\Tau} \bm\alpha_i^{(k_i)} - \beta_i^{(k_i)} + \left(\vv_i^{'\Tau}-\vv_i^{\Tau} \right)\bm\alpha_i^{(k_i)}\right] - \left[\vv_i^{\Tau} \bm\alpha_i^{(k_i')} - \beta_i^{(k_i')} + \left(\vv_i^{'\Tau}-\vv_i^{\Tau} \right)\bm\alpha_i^{(k_i')}\right]\nonumber\\
    = & \left[\left(\vv_i^{\Tau} \bm\alpha_i^{(k_i)} - \beta_i^{(k_i)}\right) - \left(\vv_i^{\Tau} \bm\alpha_i^{(k_i')} - \beta_i^{(k_i')}\right)\right] + \left(\vv_i^{'\Tau}-\vv_i^{\Tau} \right)\left(\bm\alpha_i^{(k_i)}-\bm\alpha_i^{(k_i')}\right) \nonumber\\
    \ge & \|\vv_i'-\vv_i\|_1 -  \|\vv_i'-\vv_i\|_1 = 0, \label{equ:case32-2}
\end{align}
where the first inequality is because $\bm\alpha_i^{(k_i)}-\bm\alpha_i^{(k_i')}\ge -1$. Eq.~\ref{equ:case32-2} means that at $\vv_i'$, only an allocation compatible with $\bm\alpha_{\shortn i}^{(k_{\shortn i})}$ would be selected. Then the only possibility of incompatibility comes from the changes in $\bm\alpha_{\shortn i}^{(k_{\shortn i})}$ due to varying $\vv_i$ as network input, which reduces to Case (I.A).

(II) In case (I), we show that for any given $\vv_{\shortn i}$, as along as we transform the bidder $i$'s menu at $\vv_{\shortn i}$, the allocation is guaranteed to be compatible. During training time, we apply the transformation to a grid of $\vv_{\shortn i}$. To close the proof, we need to prove that for $\forall \vv'_{\shortn i}$ that is not a grid point, the allocation is still compatible. To be specific, we show this for $\forall \vv'_{\shortn i}\in \mathcal{N}_{\shortn i,\frac{\epsilon}{2}}=\{\vv_{\shortn i}' | \|\vv_{\shortn i}'-\vv_{\shortn i}\|_\infty\le \epsilon / 2\}$.

For $\vv'_{\shortn i}$, we require that bidder $i$ receives the same post-transformation menu as in the case of $\vv_{\shortn i}$. This menu-level discretization will not violate DSIC as the menu is still self-bid independent and the menu selection is still agent-optimizing. To see this, a special case of this menu discretization is a global menu which is used in RochetNet.

In this way, if bidder $\shortn i$ does not change its selection in $\mathcal{N}_{\shortn i,\frac{\epsilon}{2}}$, then case (II) reduces to case (I) because bidder $i$'s selection is the same as in case (I). So the question is how to ensure that bidder $\shortn i$ does not change its selection.

Suppose that bidder $\shortn i$ selects $(\bm\alpha_{\shortn i}^{(k_{\shortn i})}, \beta_{\shortn i}^{(k_{\shortn i})})$ at $\vv_{\shortn i}$. Then at $\vv_{\shortn i}'$, for any other elements than $k_{\shortn i}$, we have:
\begin{align}
    & \left(\vv_{\shortn i}^{'\Tau} \bm\alpha_{\shortn i}^{(k_{\shortn i})} - \beta_{\shortn i}^{(k_{\shortn i})}\right) - \left(\vv_{\shortn i}^{'\Tau} \bm\alpha_{\shortn i}^{(k_{\shortn i}')} - \beta_{\shortn i}^{(k_{\shortn i}')}\right) \nonumber\\
    = & \left[\vv_{\shortn i}^{\Tau} \bm\alpha_{\shortn i}^{(k_{\shortn i})} - \beta_{\shortn i}^{(k_{\shortn i})} + \left(\vv_{\shortn i}^{'\Tau}-\vv_{\shortn i}^{\Tau} \right)\bm\alpha_{\shortn i}^{(k_{\shortn i})}\right] - \left[\vv_{\shortn i}^{\Tau} \bm\alpha_{\shortn i}^{(k_{\shortn i}')} - \beta_{\shortn i}^{(k_{\shortn i}')} + \left(\vv_{\shortn i}^{'\Tau}-\vv_{\shortn i}^{\Tau} \right)\bm\alpha_{\shortn i}^{(k_{\shortn i}')}\right]\nonumber\\
    = & \left[\left(\vv_{\shortn i}^{\Tau} \bm\alpha_{\shortn i}^{(k_{\shortn i})} - \beta_{\shortn i}^{(k_{\shortn i})}\right) - \left(\vv_{\shortn i}^{\Tau} \bm\alpha_{\shortn i}^{(k_{\shortn i}')} - \beta_{\shortn i}^{(k_{\shortn i}')}\right)\right] + \left(\vv_{\shortn i}^{'\Tau}-\vv_{\shortn i}^{\Tau} \right)\left(\bm\alpha_{\shortn i}^{(k_{\shortn i})}-\bm\alpha_{\shortn i}^{(k_{\shortn i}')}\right) \nonumber\\
    \ge &\left[\left(\vv_{\shortn i}^{\Tau} \bm\alpha_{\shortn i}^{(k_{\shortn i})} - \beta_{\shortn i}^{(k_{\shortn i})}\right) - \left(\vv_{\shortn i}^{\Tau} \bm\alpha_{\shortn i}^{(k_{\shortn i}')} - \beta_{\shortn i}^{(k_{\shortn i}')}\right)\right]  -  \epsilon/2, \label{equ:case2}
\end{align}
The first term in~\ref{equ:case2} is the utility difference between two menu elements. Similar to case (I.B), after sampling and prior to transforming, we verify whether the utility of second best menu element is smaller by at least $\epsilon/2$ than that of the best element. If it is not, we add a new grid point to reduce $\epsilon$ to $\epsilon/2$. This procedure can be repeated until the condition is met. Once the condition is satisfied, bidder $\shortn i$ would note change its selection in $\mathcal{N}_{\shortn i,\frac{\epsilon}{2}}$.
% We also note that the condition of adding a new grid point in case (I.B) and (II) can be relaxed by replacing the \emph{second best menu element} by the \emph{best incompatible menu element}, as bidder $\shortn i$ can always choose a compatible element with in
\end{proof}

% (II) Case 2: Bidder $i$ changes its menu element selection in \neighbor. In this case, we prove that bidder $i$ would only choose menu elements that are compatible with bidder $\shortn i$'s choice.

% For $\forall \vv_i'\in$ \neighbor, it is easy to find a subset of samples $\mathcal{V}_i'=\{\vv_i^{\ell_1}, \vv_i^{\ell_2},\cdots,\vv_i^{\ell_m}\}$ used in the transform, so that $\vv_i'$ can be expressed as a linear combination of samples in $\mathcal{V}_i'$:
% \begin{align}
%     \vv_i' = \sum_{s=1}^{m} a_s \vv_i^{\ell_s}; \ \ \sum_{s=1}^{m} a_s=1;\ \  \forall s,\ a_s\in[0,1].
% \end{align}
% We prove by contradiction and assume that at $\vv_i'$ bidder $i$ selects menu element $(\bm\alpha_i^{(k)}, \beta_i^{(k)})$ that is 


% \begin{table} [t]
%     \caption{Yao.}\label{tab:yao_scale_up_bidder}
%     \centering
%     \begin{tabular}{CRCRCRCRCRCRCR}
%         \toprule
%         \multicolumn{2}{c}{\multirow{2}{*}{}} &
%         \multicolumn{2}{l}{\multirow{2}{*}{Alg.}} &
%         \multicolumn{2}{l}{\multirow{2}{*}{Perf.}} &
%         \multicolumn{8}{c}{Setting}\\
        
%         \cmidrule(lr){7-14}
%         \multicolumn{2}{c}{} &
%         \multicolumn{2}{l}{} &
%         \multicolumn{2}{l}{} &
%         \multicolumn{2}{c}{(3, 3, 4, 0.3)} & 
%         \multicolumn{2}{c}{(5, 3, 4, 0.3)} & 
%         \multicolumn{2}{c}{(7, 3, 4, 0.3)} & 
%         \multicolumn{2}{c}{(10, 3, 4, 0.3)}\\
%         \cmidrule(lr){1-2}
%         \cmidrule(lr){3-4}
%         \cmidrule(lr){5-6}
%         \cmidrule(lr){7-8}
%         \cmidrule(lr){9-10}
%         \cmidrule(lr){11-12}
%         \cmidrule(lr){13-14}
        
%         \multicolumn{2}{c}{\multirow{4}{*}{Ours}} & \multicolumn{2}{l}{\multirow{2}{*}{Before Transf.}}  & \multicolumn{2}{l}{Feas.} & \multicolumn{2}{l}{100\%} & \multicolumn{2}{l}{100\%} & \multicolumn{2}{l}{100\%}  & \multicolumn{2}{l}{100\%} \\
%         \multicolumn{2}{c}{} & \multicolumn{2}{l}{}  & \multicolumn{2}{l}{Rev.} & \multicolumn{2}{l}{7.82202u..} & \multicolumn{2}{l}{9.1435} & \multicolumn{2}{l}{7.4735} & \multicolumn{2}{l}{6.7186} \\
%         \cmidrule(lr){3-4}
%         \cmidrule(lr){5-6}
%         \cmidrule(lr){7-8}
%         \cmidrule(lr){9-10}
%         \cmidrule(lr){11-12}
%         \cmidrule(lr){13-14}
%         \multicolumn{2}{c}{} & \multicolumn{2}{l}{\multirow{2}{*}{After Transf.}}  & \multicolumn{2}{l}{Feas.} & \multicolumn{2}{l}{100\%} & \multicolumn{2}{l}{100\%} & \multicolumn{2}{l}{100\%} & \multicolumn{2}{l}{100\%}  \\
%         \multicolumn{2}{c}{} & \multicolumn{2}{l}{}  & \multicolumn{2}{l}{Rev.} & \multicolumn{2}{l}{\textbf{7.8309}} & \multicolumn{2}{l}{\textbf{9.1504}} & \multicolumn{2}{l}{\textbf{7.4774}} & \multicolumn{2}{l}{\textbf{6.72205}} \\
%         \midrule
%         \multicolumn{2}{c}{\multirow{5}{*}{Baselines}} & \multicolumn{2}{l}{VCG} &  \multicolumn{2}{l}{Rev.} & \multicolumn{2}{l}{9.9221} & \multicolumn{2}{l}{7.9668} & \multicolumn{2}{l}{6.9815} & \multicolumn{2}{l}{6.4908}\\
%         \multicolumn{2}{c}{} & \multicolumn{2}{l}{Item-Myerson} & \multicolumn{2}{l}{Rev.} & \multicolumn{2}{l}{10.9220} & \multicolumn{2}{l}{7.2829} & \multicolumn{2}{l}{5.4607} & \multicolumn{2}{l}{4.5490}\\
%         % \multicolumn{2}{c}{} & \multicolumn{2}{l}{Lottery AMA} & \multicolumn{2}{l}{Rev.} & \multicolumn{2}{l}{} & \multicolumn{2}{l}{\textbf{}} & \multicolumn{2}{l}{\textbf{}} & \multicolumn{2}{l}{} & \multicolumn{2}{l}{\textbf{}}\\
%         \multicolumn{2}{c}{} & \multicolumn{2}{l}{AMenuNet} & \multicolumn{2}{l}{Rev.} & \multicolumn{2}{l}{10.2852} & \multicolumn{2}{l}{8.1416} & \multicolumn{2}{l}{7.0697} & \multicolumn{2}{l}{6.5349}\\
%         \cmidrule(lr){3-4}
%         \cmidrule(lr){5-6}
%         \cmidrule(lr){7-8}
%         \cmidrule(lr){9-10}
%         \cmidrule(lr){11-12}
%         \cmidrule(lr){13-14}
%         \multicolumn{2}{c}{\multirow{2}{*}{}} & \multicolumn{2}{l}{\multirow{2}{*}{RegretNet}} & \multicolumn{2}{l}{Rev.} & \multicolumn{2}{l}{12.8052} & \multicolumn{2}{l}{9.17377} & \multicolumn{2}{l}{7.50169} & \multicolumn{2}{l}{6.6799}\\
%         \multicolumn{2}{c}{} & \multicolumn{2}{l}{} & \multicolumn{2}{l}{IC Viol.} & \multicolumn{2}{l}{0.00951} & \multicolumn{2}{l}{0.00846} & \multicolumn{2}{l}{0.00548} & \multicolumn{2}{l}{0.00943} \\
%         \cmidrule(lr){1-2}
%         \cmidrule(lr){3-4}
%         \cmidrule(lr){5-6}
%         \cmidrule(lr){7-8}
%         \cmidrule(lr){9-10}
%         \cmidrule(lr){11-12}
%         \cmidrule(lr){13-14}
%         \multicolumn{2}{c}{
%         \multirow{3}{*}{Ablations}} &  \multicolumn{2}{l}{Ours} & \multicolumn{2}{l}{Rev.} & \multicolumn{2}{l}{} \\
%         \multicolumn{2}{c}{} & \multicolumn{2}{l}{Ours} & \multicolumn{2}{l}{Rev.} & \multicolumn{2}{l}{} & \multicolumn{2}{l}{\textbf{}} & \multicolumn{2}{l}{\textbf{}} & \multicolumn{2}{l}{}  \\
%         \multicolumn{2}{c}{} & \multicolumn{2}{l}{Ours} & \multicolumn{2}{l}{Rev.} & \multicolumn{2}{l}{} & \multicolumn{2}{l}{\textbf{}} & \multicolumn{2}{l}{\textbf{}} & \multicolumn{2}{l}{}  \\
%         \toprule
%         \multicolumn{2}{c}{Optimal} & \multicolumn{2}{l}{\citet{yao2017dominant}} & \multicolumn{2}{l}{Rev.} & \multicolumn{2}{l}{\textbf{7.8309}} & \multicolumn{2}{l}{\textbf{9.1504}} & \multicolumn{2}{l}{\textbf{7.4774}} & \multicolumn{2}{l}{\textbf{6.72205}} \\
%         \toprule
%     \end{tabular}
% \end{table}


Introduction paragraph on why not LP.
Our MILP model for price adjustment presents several advantages over automatic mechanism design approaches using linear programming for designing auctions. (1) Deep learning offers efficient initial solutions, allowing us to significantly reducing the complexity of the MILP models.  \dcp{i don't find this prev sentence compelling---if we need a massive number of vars, then having `good initialization` doesn't obviously help}
%
We identify two particularly useful features that typically reduce >80\% of binary variables in MILP models. \dcp{`reduce`?}
 Firstly, within the network-generated menus, we observe that it is typical for only
 two or three elements to be preferred by a bidder over the IR choice. \dcp{`IR choice`?} 
We can restrict price changes to be positive \dcp{i.e., increasing prices? also, use `price` not `payment` for the menu choices ... it only becomes payment when it is actually collected from a bidder} so that the elements with negative utilities cannot become better than the IR choice after transformation, which means binary variables associated with these elements can be eliminated. Additionally, given the already low incompatibility rate at the end of training,
 the ``big-M method" is not necessary for every compatible sample. \dcp{`every compatible sample` not clear, and also before saying it's not necessary you need to say what it is used for...}
%
Rather, a simple linear constraint ensuring bidders retain their choices is sufficient. \dcp{make this more clear} (2) The MILP approach leaves undisturbed the allocation elements of a bidder's menu and just adjusts the prices associated with each element, which  further decreases computational complexity. \dcp{as per our conversations, we'll prob rewrite this to note that LPs are not DSIC. I do think we should  consider stating in intro the main scaling analysis in terms of number of agents, number of items, and Lipschitz constant for our method.}



'






\dcp{following discussion is unclear. what is this mention of supervised learning, freezing, etc? i made an earlier comment on this in prev section: we need to explain how the transforms are generalized across the entire value domain and then stick with this method in this proof} 
If we do not train the network by supervised learning to remember the price adjustments, we can choose to freeze the menu in \neighborjoint. Note that this would not violate the DSIC guarantee of our method, because the menu is still self-bid independent. The extreme of this discretized menu scheme is RochetNet that uses a constant menu. A locally constant menu in \neighborjoint~would affect the discussion of case (I). Now the utility change of any menu element (Eq.~\ref{eq:change_gap}) is upper bounded by $\epsilon/2$, which is the maximum changes in $\vv_i$. Therefore, according to Eq.~\ref{eq:no_vio_1}, we can have a safety margin $s_m=\epsilon$ to ensure that the bidders would not change their menu selection in \neighborjoint.








(Sketch) We first prove 
 by backward induction
 that the aggregate allocation of bidders at any grid point
is at most $1-n\cdot s_f$.

(Base Step) For bidder ($n-1$), the criterion for identifying  a feasible menu elements (Eq.~\ref{equ:multi_mip_feas_standard}) is the same as in the two-bidder case except for a larger safety margin ($n\cdot s_f$). Since the rest of the MILP is unchanged,
 we know that the aggregate allocation of bidder ($n-1$) and $n$ is at most $1-n\cdot s_f$.

(Inductive Step) For bidder $i<n-2$, from induction, we know that $\min\left(1, \sum_{j=i+1}^n\bm\alpha^*_{j}(\vv_{\shortn j}) \right)$ in Eq.~\ref{equ:multi_mip_feas_standard} is $\sum_{j=i+1}^n\bm\alpha^*_{j}(\vv_{\shortn j})$, and thus the transformation ensures that bidder $i$ will not select elements that make the aggregate allocation (including bidder $i$) larger than the right hand side of Eq.~\ref{equ:multi_mip_feas_standard}, which is $1-n\cdot s_f$. This finishes the proof.

==> text/1-Introduction-SATS.tex <==
\section{Introduction}

%dcp cut Standard auctions rarely allow bidders to express such non-additive preferences. Emerging to address this shortcoming, %so that more intricate valuation structures could be accommodated. 

When selling multiple items simultaneously, bidders may have complex valuations that exhibit synergies among items. For instance, some items may act as complements, making their collective value to a bidder exceed the sum of their individual values. \emph{Combinatorial auctions} (CAs) support these kinds of valuations by allowing bids on bundles of items. The need for such auctions was recognized as early as 1922~\cite{uscongress1925e}, and their formal definition dates to 1982~\cite{rassenti1982combinatorial}, where they are exemplified in the allocation of congested airport runways. Since then, CAs have proven pivotal in addressing a wide range of real-world challenges, most notably in the auctioning of spectrum licenses~\cite{cramton1997fcc,palacios-huerta24}--efforts whose far-reaching impact contributed to the awarding of the 2020 Nobel Prize in Economic Sciences~\cite{NobelPrizeEcon2020}.

Despite their  prominence, designing optimal CAs remains fundamentally challenging. As with auctions for additive or unit-demand valuations, it is typical to seek mechanisms that are (1) dominant-strategy incentive compatible (DSIC, also strategy-proof), ensuring that bidders benefit most by reporting their true values, and (2) revenue-maximizing from the auctioneer's perspective. However, even the seemingly simpler single-bidder combinatorial setting---a foundational building block for multi-bidder scenarios---still lacks a comprehensive theoretical characterization. This gap highlights the broader difficulty in developing and analyzing optimal mechanisms for general CAs.

In response to similar theoretical obstacles in additive and unit-demand valuations, researchers have explored deep learning techniques, commonly referred to as \emph{differentiable economics}~\cite{dutting2024optimal}. In particular, deep menu-based methods show promise. These methods learn a menu of options for a bidder, guaranteeing strategy-proofness, provided the menu remains self-bid independent and agent-optimizing~\citep{hammond1979straightforward}. 
For a CA, each option in a menu will correspond to a bundle of items (or distribution on bundles) and a price. Following {\em RochetNet}~\cite{dutting2024optimal}, various methods have been developed for the single-bidder but non-combinatorial setting~\cite{curry2022differentiable,duan2023scalable,shen2019automated,dutting2024optimal}, demonstrating
the ability to rediscover auctions that are provably optimal. {\em GemNet}~\cite{wang2024gemnet} extends menu-based methods to multi-bidder scenarios and pushes the frontier for the design of multi-item auctions with additive or unit-demand
valuations. 
%These findings may inspire theoretical work by illuminating mechanisms conjectured to be optimal.
%Moreover, 
%%
%Second, both theoretical and empirical studies encounter bottlenecks. Theoretically, mechanisms for the general CA setting with %provably optimized revenue are still elusive. Empirically, as we will analyze,

Unfortunately, differentiable economics has made only limited headway on the problem of optimal CA design and the fundamental challenge of handling the exponential number of bundles remains largely untouched. \citet{dutting2024optimal} deal with two items, and with a learned mechanism that does not guarantee exact DSIC. \citet{duan2024scalable} scale to 10 items, but restrict their attention to  the virtual valuation combinatorial auction (VVCA), which is not a fully general design space. Neither paper provides a path towards \twadd{DSIC and expressive mechanisms for} tens or hundreds of items, 
which presents a formidable obstacle and necessitates the development of novel methodology.
%

Focusing on the single-bidder setting, we make progress by developing a menu-based, deep learning method for \twadd{DSIC and expressive} CAs that scales to as many as 
150 items.   Single-bidder CAs, although less general than multi-bidder CAs, are applicable to  real-world problems. Consider  a digital content provider offering a collection of movies to a viewer, a cloud computing vendor offering different features (clock speed, number of compute units,  background execution, etc.), a monopolist seller offering  highly complementary patents to a  pharmaceutical firm, or a utility  supplier bundling electricity, gas, and renewable energy for an industrial customer. In these examples, the buyer's valuation may be influenced by strong complementarities or substitutes across items.
%, and the seller may seek to  optimize revenue. 
Moreover, and as discussed in Section~\ref{sec:multi-bidder}, 
this single-bidder deep mechanism design algorithm, which uses generative models to solve
the bundle scalability issue, provides a 
direction towards the automated design of multi-bidder CAs at scale.
%
% highlighting that the single-bidder case is an essential domain for refining our understanding of combinatorial auctions.

\begin{figure}
    \centering
    \includegraphics[width=\linewidth]{figures/idea.pdf}
    \caption{(a) A menu for additive or unit-demand valuations only needs to specify allocation probabilities for each item. However, item-wise allocation probabilities are  too inflexible
   % ambiguous
    for CAs, as bidder values are specified for bundles. (b) The space complexity for representing an explicit distribution on bundle-wise allocations grows exponentially with the number of items. (c) We represent a bundle distribution
    through a tractable initial distribution and an ordinary differential equation (ODE). 
    % \dcp{don't capitalize Ord Diff Eq in subtitle (c)}
    \label{fig:idea}}
\end{figure}
To understand the challenge of optimal CA design, 
%see why the complexity of mechanism design remains significant even in the absence of competition among multiple bidders, 
%
even with one bidder, 
Fig.~\ref{fig:idea} compares  menus for additive and unit-demand valuations with menus for combinatorial valuations.
For an additive bidder, it suffices to specify in a menu element (or option) the \emph{item-wise allocation probabilities} such as $[0.3, 0.4, 0.6]$ along with a price. A bidder's  expected value for the corresponding menu element can be calculated as the weighted sum of item values. A similar, item-wise  approach also works for a unit-demand bidder.
However, such item-wise allocations are ambiguous in CAs.
For example, $[0.3, 0.4, 0.6]$ could be $0.3[1,0,0]+0.4[0,1,0]+0.6[0,0,1]$ or
$0.3[1,1,1]+0.1[0,1,1]+0.2[0,0,1]$, with the same item-wise allocation  decomposed as different \emph{bundle-wise allocations}, leading to conflicting valuations. One could predefine how to interpret a marginal item-wise allocation to avoid ambiguity, for example adopting the product distribution semantics. However, our experiments show that learning product distributions (\eg, \bundle~in Table~\ref{tab:exp_results})  lags behind some fixed-allocation menus. A product distribution also requires computation that is exponential in the number of items to evaluate the value for a bidder with a general, combinatorial valuation function. 
Moreover, the use of a product distribution lacks flexibility; e.g.,  $0.5[1,1,0]+0.5[0,0,1]$ cannot be represented as a product distribution. Indeed, any fixed mapping from the $m$-dimensional space \twadd{($m$ is the number of items)} of item-wise allocations to the $2^m$-dimensional space of bundle-wise allocations means that many bundle-wise allocations are left uncovered.
%\dcp{this is where we'd like to add a FN to point to an example from the theoretical literature of the need for non-product bundle distributions for rev optimality. I don't think we have one.} \tw{In case we cannot find such a reference. What about this:} \twadd{... One could predefine how to interpret a marginal item-wise allocation to avoid ambiguity, for example adopting the product distribution semantics. However, such interpretations require computation that is exponential in the number of items to evaluate the value for a bidder with a general, combinatorial valuation function. More importantly, these interpretation lacks flexibility; e.g.,  $0.5[1,1,0]+0.5[0,0,1]$ cannot be represented as a product distribution. While there is no theoretical investigation on the optimality of these marginal distributions in CAs, our experiments show that learning product distributions (\eg, \bundle~in Table~\ref{tab:exp_results}) even lags behind some fixed-allocation menus. The essence of this problem is that a predefined interpretation specifies a mapping from the $m-$dimensional space of item-wise allocations to the $2^m$-dimensional space of bundle-wise allocations. This exponential dimensionality difference means that not all bundle-wise allocations can be covered by such a mapping. [The end of this para.]} \tw{I changed the order of these two problems because the next para starts with "expressiveness". I also changed the sentence order, in hope that the last sentence can explain a little bit about why product distributions might not give optimal results, in case there is no theory.}
% \dcp{I suggest this slightly simpler phrasing,  which does not state explicitly there is no theory.}
%\dcp{I've come to think about this a bit differently. It's not the ambiguity that's a problem. One can make it non ambiguous by saying, for example, this is a product distribution.  Rather, there is a lack of expressiveness/flexibility and a challenge with complexity, avoiding needing to evaluate over an exponential number of bundles.}

One way to achieve expressiveness would be to explicitly specify, for each menu element, an allocation probability for each possible bundle, as shown in Fig.~\ref{fig:idea} (b). But the number of bundles grows exponentially with the number of items, making it intractable to learn these bundle-wise allocations. \twadd{Aside from menu-based approaches,} other state-of-the-art deep learning methods for mechanism design face a similar challenge: they do not suggest a way to represent bundle-wise allocation distributions efficiently and flexibly.
%such as RochetNet \twadd{and RegretNet}~\cite{dutting2024optimal}%with an explicit, enumerative representation. 
%\dcp{not following the intent of this prev sentence. is it getting at AMAnet, RegretNet, etc?} \tw{Yes. In the figure, we discuss menu-based methods. I want to say that other methods like RegretNet also face similar questions.}
%

%
% Bundle distributions matter when we calculate the utility of menu elements, which is the sum of bundle values weighted by bundle allocation probabilities.
%\dcp{I think the connection between $\vs_0$ and $\vs_t$ is conceptually confusing. Do we think about applying this transform to any $\vs_0$ in $\mathbb{R}^m$, with $\vs_t$ here really being the $\vs_t$ that ``is generated from applying the ODE to $\vs_0$"; that is, is this really $\vs_t(\vs_0)$, where we don't write it this way because it would be too cumbersome?} 

In this paper, we solve this problem by avoiding the need to directly represent and learn an exponential-dimensional specification of a distribution on bundles. Instead, we represent a distribution on bundles by a tractable and low-dimensional \emph{initial distribution}, $\alpha_0(\vs_0)$, on {\em initial bundle variables}, $\vs_0\in \mathbb{R}^m$,
and an ordinary differential equation (ODE): $d\vs_t = \varphi(t, \vs_t) dt$. The ODE operates on \emph{bundle variables}, $\vs_t\in\mathbb{R}^m$, through the {\em vector field} $\varphi(t, \cdot)$. Here $m$ is the number of items and $t\in[0,T]$ is the {\em ODE time}. A feasible bundle corresponds to a bundle variable where the entries are all 0s or 1s. Formally, $\vs_t$ is generated from a sample $\vs_0$ by applying the ODE: $\vs_t(\vs_0)=\vs_0+\int_0^t \varphi(\tau,\vs_\tau) d\tau$. We omit the dependence on $\vs_0$ and write $\vs_t$ for simplicity.
In this way, the ODE transforms the initial distribution $\alpha_0(\vs_0)$ to a final distribution $\alpha_T(\vs_T)$ at time $T$. The idea is to (1) train the vector field so that the support of the final distribution $\alpha_T(\vs_T)$ corresponds to feasible bundles; (2) fix this trained vector field $\varphi(t, \cdot)$, and learn a different initial distribution $\alpha_0(\vs_0)$ (therefore a different final distribution over bundles) and price for each menu
element, so that the menu maximizes expected revenue. 
\if 0
\dcp{clarify: I think it operates on the distribution by transforming the random variable $\vs_t$. is this the right
way to think about it?}
\dcp{add something like `A feasible bundle corresponds to a bundle variable where the entries are all 0s or 1s.`}.
\dcp{should we say something like $\vs_T$ is the random variable corresponding to 
the bundle variable at time $T$?}
\tw{This para has been reworked. Hope it can resolve the concerns.}
The generation of the final distribution is governed by the ODE. 
\fi


\begin{figure}
    \centering
    \includegraphics[width=\linewidth]{figures/flow_init.png}
    \caption{Evolution of the vector field $\varphi$ during the first stage of menu training: \emph{Flow Initialization}. The x- and y-axes represent the bundle variables for two of items. $x=1$ means item A is in the bundle, and $y=1$ means item B is in the bundle. We employ an ODE $d\vs_t = \varphi(t, \vs_t) dt$ to generate the final distribution $\alpha_T(\vs_T)$ (a distribution over bundles), represented by blue dots, from a simple initial distribution $\alpha_0(\vs_0)$, represented by green dots. During the first stage, $\alpha_0(\vs_0)$ is fixed as a mixture-of-Gaussian distribution. Dot opacity represents probability density. The aim of this first stage is to train the vector field so that the final distribution has all feasible bundles as its support (see Sec.~\ref{sec:viz}).
    \label{fig:flow_init}}
\end{figure}
This method draws inspirations from generative AI models, such as {\em diffusion models}~\cite{ho2020denoising, kadkhodaie2023generalization,song2021score,song2019generative} and, in particular, {\em flow matching}~\cite{chen2018neural,liu2022flow,lipman2022flow}.  We thus call the  method \name~to emphasize the core idea of using flow matching to model bundle distributions. Prior work has successfully shown how to transform simple distributions such as the Gaussian distribution to complex \emph{target distributions} such as natural images~\cite{rombach2022high,esser2024scaling}, language~\cite{lou2024discrete}, and videos~\cite{stabilityAI2023}. In these generative AI tasks, the target distribution is known and observed as the data distribution in large-scale pre-training datasets. Our technical novelty is to extend generative models to solve optimization problems, seeking a bundle distribution (and price) for
each menu element that optimizes expected revenue. 
There is no known target distribution in our work.
%\dcp{somewhere in paper explain how novel these uses of 
%diffusion nets for combinatorial objects such as bundles are -- what is the technical innovation?}\tw{Add such an explanation here.}

% Unlike these kinds of generation models,  we face an optimization problem and with no known final distribution as a prior. 
% \dcp{`with no known final distribution as a prior` unclear}
% Nevertheless, as is standard in this literature, we say the ODE induces a \emph{flow} $\phi_t(\vs_0)$ that gives  solution to the ODE at time $t$.  \dcp{connection between `flow`, vector field, and distribution $\alpha_T$ unclear, also why `Nevertheless`}


Central to our method is that the distribution's evolution under the ODE
is governed by the {\em Liouville equation}~\cite{liouville1838note}:
%
\begin{align}
    \log \alpha_t(\vs_t) = \log \alpha_0(\vs_0) -\int_0^t \nabla\cdot\varphi(t, \vs_t) dt.\label{equ:demo_liouville}
\end{align}
We carefully design the functional forms of the vector field $\varphi(t, \cdot)$ so that the integral of its divergence $\nabla\cdot\varphi(t, \cdot)$ is easy to compute, thereby allowing efficient menu optimization. As the first stage of menu learning, we fix the initial distribution $\alpha_0(\vs_0)$ to a mixture-of-Gaussian distribution 
and train a single vector field $\varphi(t, \cdot)$ to transport any initial variable $\vs_0$ to a feasible bundle at final time $T$. An illustration of how the vector field evolves during this first training stage is shown in Fig.~\ref{fig:flow_init}.
%\tw{I add this para back with more details. I think it is important as it describes the first step of menu training and some novelties.}

\begin{figure}
    \centering
    \includegraphics[width=\linewidth]{figures/flow_train.png}
    \caption{Visualization of the second stage of training: \emph{Menu Optimization}. The figure presents snapshots of four menu elements (organized in columns) at different training iterations (organized in rows), showing the bundle distribution and price for each element, along with the test-time auctioneer revenue from the entire menu at the corresponding iteration. The x- and y-axes represent the bundle variables for two of items. $x=1$ means item $A$ is in the bundle, and $y=1$ means item $B$ is in the bundle. We fix the vector field (blue curves) and update initial distributions of elements to manipulate distributions over bundles (refer to Sec.~\ref{sec:viz}).% \dcp{typo, revenue in bottom row? its the same for every element.} \tw{they are revenue of the menu :)} \dcp{but then why are the rev numbers different in each column for other rows? i thought you were showing the per-element revenue.} \tw{Because train iterations are different for other rows. E.g., we have iteration 450, 270, 150, 210 in the 3rd row (I selected critical changes during training, and they happen at different times). Only the last row has the same iteration.}
    \label{fig:flow_train}}
\end{figure}

%\dcp{[this gives a menu element]} 
With this vector field fixed, as a second stage we then train each element in a menu so that the menu maximizes expected auction revenue.  The advantage of our flow-based method is that, \twadd{during both training and testing}, we can efficiently calculate the utility of each menu element $k$ by substituting the bundle distribution $\alpha_T^{(k)}(\vs_T)$ with $\alpha_0^{(k)}(\vs_0)$ as described in Eq.~\ref{equ:demo_liouville}.
We re-parametrize the initial distribution $\alpha_0^{(k)}(\vs_0)$ so that the resulting bundle distribution, $\alpha_T^{(k)}(\vs_T)$, becomes trainable.
To ensure DSIC, we design the initial distribution $\alpha^{(k)}_0(\vs_0)$ to have finite support. Specifically, we use mixture-of-Dirac distributions.
This enables precise reconstruction of the bundle distribution $\alpha_T^{(k)}(\vs_T)$ and thus the utility of a menu element by enumerating the support of $\alpha_0^{(k)}(\vs_0)$.

For optimization, each menu element shares a common vector field and has separate trainable parameters for its price and  initial distribution (mixture weights and support points of the mixture-of-Dirac distribution).  
The gradients of the revenue-maximizing loss backpropagate through the ODE back to parameters of $\alpha_0^{(k)}(\vs_0)$, guiding updates that increase expected revenue. 
As a demonstration of  this second stage, we illustrate changes of the initial distribution and corresponding bundle  distribution for each of four different menu elements, as well as corresponding prices and auction revenue in Fig.~\ref{fig:flow_train}. 
%\dcp{do we actually use mixture-of-Dirac in second stage? Is it clearer if explained this way?} \dcp{suggest using $^{(k)}$ through this paragraph to distinguish from the initial distribution used in the first stage} \tw{I changed the sentence order and add some transitions to make this part clearer.}

% we set an almost-zero variance in the components of the mixture-of-Gaussian distributions, effectively making them behave like
% \tw{or mixture weights and means of the narrow mixture-of-Gaussian distribution}
% (we will make use of the , but other distributions like a mixture-of-Dirac also work).  , %\dcp{will be a bit confusing, given we talk about mix-of-gaussian. worth a footnote to clarify the basic idea for how it becomes, in effect, finite?}%

%In principle, our method enjoys full expressiveness when the support size of the initial distribution is comparable to the number of bundles.
Although the number of bundles in the support of the bundle distribution $\alpha^{(k)}_T(\vs_T)$ for menu element $k$ is 
at most the size of the support of the initial distribution $\alpha^{(k)}_0(\vs_0)$, what this representation achieves
is that the bundle distribution $\alpha^{(k)}_T(\vs_T)$ can be flexibly learned.
In practice, we observe that even a small support size for bundle distribution $\alpha^{(k)}_T(\vs_T)$ yields strong performance across various settings. Moreover, the formulation of our method does not rely on any  assumptions regarding the bidder's valuation function, for example that the valuation function can be represented on a small number 
of bundles, and thus exhibits flexibility, applicable to a large range of CA problems.
%We then conduct comprehensive experiments to thoroughly validate these attributes.
%
%\dcp{add a couple more sentences to emphasize flexibility/expressiveness}
%

We evaluate \name~using single-bidder instantiations of 
two widely recognized CA testbeds: CATS \citep{leyton2000towards} and SATS \citep{weiss2017sats}. Given the absence of established deep methods capable of extending to the settings considered in this paper, we benchmark against the following baselines. (1) \bundle: An adaptation of RochetNet~\cite{dutting2024optimal} with a menu of item-wise allocations \twadd{(and prices)} that interprets item-wise allocations as product distributions. (2) \bigbundle: This baseline fixes allocations in all menu elements, favoring bundles with the highest item counts. Prices are learned using the same gradient-based method as in RochetNet. (3) \smallbundle: Similar to \bigbundle\ but in addition to the grand bundle, which includes all items, also includes bundles with minimal item allocations. (4) \grandbundle: Employs grid search to determine a price for the grand bundle. In all cases, the menu element with the largest utility, if non-negative, is assigned to the bidder. 
%The bidder is always assigned this bundle if their utility is non-negative. 
These baselines represent progressively restrictive constraints on the flexibility of menus.

Experimental results demonstrate that our method consistently and significantly outperforms all baselines across all benchmark settings and scales effectively to auctions involving up to 150 items. Specially, for auctions with 50 to 150 items, \name~achieves 1.2-3.6$\times$ higher revenue. The training time is also considerably reduced: our method converges 1.3-21.4$\times$ faster than the deep learning baselines. A critical observation is noted when we vary the support of initial distributions, $D$, from 2 to 1. This change leads to a considerable drop in revenue in \name--up to a halving of revenue at its most severe. Since when $D=1$ each menu element deterministically assigns a single bundle, these results underscore the importance of allowing randomized distributions over bundles in differentiable economics for CA settings, a capability uniquely enabled by our methods.
% \dcp{excepting \grandbundle\ presumably! also, this is a bit susprising to me for \bigbundle\ and \smallbundle. \bundle\ doesn't surprise me.}

% Since its release in 2000, CATS has served as the standard benchmark in CA research, including five tasks inspired by economically motivated, real-world scenarios. In the two decades following CATS, spectrum auctions have emerged as a pivotal application of CAs, and SATS models settings tailored to the specific challenges of spectrum auctions. 

% These results show the flexibility, effectiveness, and scalability of \name.


% While our work primarily focuses on the traditional combinatorial auction setting rather than spectrum auctions, we conducted experiments using both CATS and SATS to comprehensively evaluate our method.
% specific applications

==> text/5-Experiments-SATS.tex <==
\section{Visualization on a didactic example}\label{sec:viz}

We present an example to visualize the training process of our method. For this, we adopt the \texttt{Regions} environment from the CATS testbed and consider uniform distributions with five items. 

Fig.~\ref{fig:flow_init}, already presented in the paper, shows the learning effect of Stage 1. Specifically, we fix the initial distribution and update the vector field. For the flow network architecture, the $Q$ and $\sigma$ networks have three and two 128-dimensional, tanh-activated, fully-connection hidden layers, respectively. We use the Adam optimizer with a learning rate of $5e\shortn 3$ to train these networks with $20$K samples for $60$K iterations.

The x- and y-axis of Fig.~\ref{fig:flow_init} are the bundle variables for the 3rd and 4th items, respectively. $x=1$ means that the 3rd item is in the bundle, and $y=1$ means the 4th item is in the bundle. The blue lines represent the vector field, and the blue dots represent the final distribution. We can see that the vector field gradually learns to cover all possible bundles in this projected, two-item subspace, 
as indicated by points $(0,0)$, $(0,1)$, $(1,0)$, and $(1,1)$ in the plots.

Fig.~\ref{fig:flow_train} illustrates the dynamics of Stage 2. In this demonstrative example, the support size of initial distributions is set to 256. The figure is organized into four columns, each displaying changes in the bundle allocation (depicted by blue dots) and  price of a distinct menu element. Additionally, the total revenue at the corresponding training iteration (during test time) is  presented. Changes in the bundle distribution for a menu element result from updates to the initial distribution for the menu element. For the initial distributions, the positions of green dots represent the means ($\bm\mu_d^{(k)}$) of the mixture-of-Dirac components, while their opacities indicate the weights ($w_d^{(k)}$) of these components. We observe that each menu element learns to allocate different bundles. For example, Menu Element 3 manages bundles $(0,1)$ and $(1,0)$, and sets a price of 88.245 after Train Iteration 1020, at which point the revenue reaches 64.31.

\section{Experiments}

% \tw{} Use \verb|\bundle| to refer Bundle-RochetNet, \verb|\smallbundle| for Small-Bundle, and \verb|\bigbundle| for Near-Grand-Bundle, and \verb|\grandbundle| for Grand-Bundle
% At a high level \citep{catshardness}, \texttt{Regions} models an auction for real estate, or more broadly, for goods where two-dimensional adjacency determines complementarities. 
% \texttt{Regions} extends the concept of \texttt{Regions} by removing the planarity constraint, capturing arbitrary complementarities between discrete goods such as electronic components or collectibles. \textit{paths} represents an auction for transportation links between cities, or more generally, for edges in a nearly planar graph. \textit{matching} represents auctions for airline takeoff and landing rights, akin to those considered by the FAA. Finally, \textit{scheduling} models a distributed job-shop scheduling environment.
% and do not involve different types of bidders (e.g., National versus Regional bidders) - a distinction not applicable in our single-bidder setting.
% marginal allocations using the , which is commonly used to re-parameterize categorical distributions. Specifically, for an item-wise allocation $\alpha\in\mathbb{R}^m$ of a menu element, this trick will return a vectorized bundle in $[0,1]^m$, where the item $i$ is in this bundle with probability $\alpha_i$, the $i$th dimension of $\alpha$.  to $\alpha$. 
% (2) \textbf{\bigbundle}: Fixed allocations include the grand bundle and bundles close to it, prioritizing those with the most items allocated. When the menu size is insufficient to include all bundles with a certain number of items, bundles are selected randomly. For instance, with 3 items and a menu size of 3, the menu would include $[1,1,1]$ (grand bundle) and a random subset of bundles containing $n-1$ items, such as $[1,1,0]$ and $[0,1,1]$. Although we randomly select this subset, one can predefine it.
% to \bigbundle, but includes the grand bundle and bundles with minimal item allocations, starting from single-item allocations. When the menu size exceeds the number of available single-item bundles, additional bundles are included by incrementally increasing the number of allocated items. For example, with 3 items and a menu size of 5, the selected bundles would include $[1,1,1]$ and single-item bundles such as $[1,0,0]$, $[0,1,0]$, $[0,0,1]$, and $[1,0,1]$.

\begin{table}[t]
    \caption{Revenue comparison on CATS across different environments, distributions, and numbers of items. Note that \emph{when $m=10$, the menu size is large enough to accommodate all possible bundles in a menu.} \label{tab:exp_results}}
    \vspace{-0.5em}
    \centering
    \begin{tabular}{ccccccc}
        \toprule
        \textbf{Environment} & \textbf{Baseline} & $m=10$ & $m=50$ & $m=75$ & $m=100$ & $m=150$ \\
        \midrule
        \multirow{5}{*}{\makecell{CATS-Regions \\ \footnotesize Uniform Private Valuations}} 
        & \grandbundle & 162.57 & 316.27 & 321.10 & 317.00 & 314.93 \\
        & \bigbundle & \textbf{202.26} & 399.85 & 354.48 & 322.68 & 329.17 \\
        & \smallbundle & 202.16 & 322.85 & 318.33 & 326.76 & 334.20 \\
        & \bundle & 189.17 & 288.41 & 290.14 & 292.11 & 312.65  \\
        & \name & 196.19 & \textbf{555.05} & \textbf{454.96} & \textbf{390.60} & \textbf{385.68} \\
        \midrule
        \multirow{5}{*}{\makecell{CATS-Regions \\ \footnotesize Normal Private Valuations}} 
        & \grandbundle & 142.54 & 319.06 & 328.89 & 305.06 & 309.73 \\
        & \bigbundle & \textbf{181.93} & 459.97 & 405.36 & 306.60 & 312.21 \\
        & \smallbundle & 181.75 & 342.31 & 339.82 & 303.31 & 315.02 \\
        & \bundle & 167.16 & 270.23 & 300.55 & 270.23 & 291.83 \\
        & \name & 173.93 & \textbf{603.70} & \textbf{448.35} & \textbf{389.51} & \textbf{394.82} \\
        \midrule
        \multirow{5}{*}{\makecell{CATS-Arbitrary \\ \footnotesize Uniform Private Valuations}} 
        & \grandbundle & 175.09 & 329.62 & 340.40 & 343.66 & 345.98 \\
        & \bigbundle &\textbf{233.26} & 396.78 & 351.70 & 357.44 & 351.07 \\
        & \smallbundle & 222.74 & 353.20 & 355.73 & 364.33 & 360.41 \\
        & \bundle & 205.02 & 316.79 & 312.41 & 313.76 & 334.51 \\
        & \name & 211.55 & \textbf{560.71} & \textbf{467.79} & \textbf{434.77} & \textbf{420.75} \\
        \midrule
        \multirow{5}{*}{\makecell{CATS-Arbitrary \\ \footnotesize Normal Private Valuations}} 
        & \grandbundle & 186.59 & 354.86 & 345.88 & 329.99 & 336.45 \\
        & \bigbundle & \textbf{248.16} & 478.67 & 349.34 & 335.75 & 339.10 \\
        & \smallbundle & 248.13 & 376.31 & 352.80 & 343.58 & 348.39 \\
        & \bundle & 221.49 & 348.41 & 312.79 & 304.00 & 316.81 \\
        & \name & 235.80 & \textbf{646.37} & \textbf{490.03} & \textbf{428.54} & \textbf{394.37} \\
        \bottomrule
    \end{tabular}
    \vspace{-0.5em}
\end{table}
\begin{table}[t]
    \caption{Revenue comparison on SATS \texttt{Multi-Band Value Model}. \dcpadd{In addition to \name, the \grandbundle\ method is also competitive in this environment.} With $m=24$, we vary the maximum number of XOR atoms per valuation (\ie, valuation function size): $a = 10, 20, 30, 40, 50$. \jf{updated numbers, need to think about what to do with this table} \label{tab:sats}} 
    \centering
    \vspace{-0.5em}
    \begin{tabular}{ccccccc}
        \toprule
        \textbf{Environment} & \textbf{Baseline} & $a=10$ & $a=20$ & $a=30$ & $a=40$ & $a=50$ \\
        \midrule
        \multirow{5}{*}{\makecell{SATS \\ \footnotesize Multi-Band Value Model}} 
        & \grandbundle & 2580.2 & 2766.1 & 2848.4 & 2878.6 & 2917.5 \\
        & \bigbundle   & \textbf{2731.6} &  \textbf{2839.3}& 2865.1 & \textbf{2962.8 } & \textbf{3013.1}\\
        & \smallbundle & 2601.0 &  2809.9 & \textbf{2872.7} & 2941.0 & 2977.6\\
        & \bundle      & 2413.4 & 1968.8 & 2174.9 & 2234.6 & 2211.5 \\
        & \name        & 2600.3 & 2767.4 & 2860.3 & 2902.8 & 2926.5 \\
        \bottomrule
    \end{tabular}
    \vspace{-0.5em}
\end{table}

% According to the benchmark setting, \emph{there are 2400 possible bundles in total, which can be accommodated within the menus of baselines}. \dcp{but wouldn't they have to be small- or big-bundles for this to be true?}

\subsection{Testbeds}

We evaluate our method on two standard benchmarks that have been used in
CA research since 2000: CATS \citep{leyton2000towards} and SATS \citep{weiss2017sats}. 

\begin{figure}
    \centering
    \includegraphics[width=\linewidth]{figures/lc_m.pdf}
    \caption{Learning curves of \name~and baselines on \texttt{CATS Arbitrary} with normal valuation distributions with different numbers of items. The three rows are results for 50, 100, and 150 items, respectively. The three columns shows the changes of test revenue as a function of the number of training iterations, wall time in seconds, and the number of training samples, respectively. 
    % \dcp{WOW! can we also say this is representative of SATS?} \tw{I am afraid we can not. I am considering downplaying the emphasis on our advantage in training speed, and Jeff is double checking whether baselines can converge quicker.} \dcp{ok, I talked with Jeff briefly about this yesterday and understand we're taking another look at the choice of learning rate for the RochetNet baselines.}
    \label{fig:lcm}}
\end{figure}

\textbf{CATS} has five different environments: \texttt{Regions}, \texttt{Arbitrary}, \texttt{Paths}, \texttt{Matching}, and \texttt{Scheduling}. These provide stylized representations of diverse real-world problems ranging from real estate and electronic components to transportation links and airline scheduling rights. Analysis of CA winner determination problem (WDP) complexity \citep{catshardness} revealed that \texttt{Matching}, \texttt{Scheduling}, and \texttt{Paths} are considerably easier to solve than \texttt{Regions} and \texttt{Arbitrary}. The WDP complexity was measured by CPLEX runs on problems with 256 goods and 1,000 %non-dominated  dcp, dropping since we don't talk about this for our own experiments
bids, reflecting the percentage of instances where the WDP is solved within a given time frame. Therefore, as in numerous previous works that employed CATS as a benchmark \citep{gasse2019exact, hutter2009paramils, hutter2014algorithm, balcan2018learning, scavuzzo2022learning, wu2021learning, huang2023searching, song2020general, gupta2022lookback, balcan2021sample, zhang2022deep}, we focus our experiments on the challenging \texttt{Arbitrary} and  \texttt{Regions} environments. Each environment has two options for the value distribution: uniform and normal. We test both distributions with the default parameters provided by CATS.

In CATS, the valuation functions of bidders are recorded as bundle-bid pairs in an output file, with bundles from the same bidder identified by appending a dummy item tagged with a unique identifier. In effect, the bundle-bid pairs in an output file involving the same dummy item form an XOR representation of the bidder's valuation function. 
To obtain single-bidder valuations, we generate 100,000 such files and  extract valuation functions identified by a consistent dummy item. Of these, 95\% are used for training, with the remaining 5\% reserved for testing.

\textbf{SATS} is motivated by the spectrum auction domain and includes several valuation models. We focus on the Multi-Band Value Model \citep{bichler2013core}, %\tw{Maybe this is a safer way to explain:} \twadd{
as other models 
%dcp either oversimplify or 
introduce bidder types that do not align with our single-bidder framework. In the Multi-Band Value Model, 24 items are grouped into four bands. Bidder values depend on the number of allocated items in each band, with some interchangeability between items, exhibiting complements within a band while being additive across bands.
%, while bidders still bid specific bundles, not item counts. 
This setup challenges deep learning methods, as gradients may be uninformative---some changes in the bundle allocation may not affect values. As such, the Multi-Band Value Model serves to further assess the robustness of our method.
%under less-than-optimal conditions. 
% (e.g., the base value model contains only 48 bundles)
% (e.g., National vs. Regional bidders)
In SATS, the number of bidders is specified as an argument, so we directly set it to 1 to generate single-bidder valuations.

We evaluate our method with different numbers of items: 5, 10, 50, 100, and 150, across all environments and value distributions  on CATS. When varying the number of items, we set the maximum XOR atoms per bid to 5 by configuring the  \emph{maximum substitutable bids} argument. We also experiment with a fixed number of items, increasing the number of XOR atoms per valuation function in each of the CATS and SATS environments.

% we use the  setting \dcp{what does this do?} as specified in CATS, with each valuation function comprising up to five XOR atoms.

\subsection{Baselines}

Work on DSIC deep auction learning can be broadly divided into two categories. (1) Methods like AMA~\cite{curry2022differentiable,duan2023scalable} and VVCA~\cite{duan2024scalable} explore a
restricted family of affine mechanisms. Consequently, they exhibit restricted expressiveness and achieve suboptimal revenue compared to methods in the second category~\cite{dutting2024optimal}.
%\dcp{isn't solving WDPs unavoidable?}\dcp{for something like VVCA wouldn't one just have a restricted number of bundles similar to what we do? how would it be different from what we do?}\tw{I think VVCA can have these good properties, but previous work didn't realize them. Discussing these improvements might distract the readers, so I prefer to keep the discussion concise.} 
(2) Menu-based methods like RochetNet~\cite{dutting2024optimal} learn an item-wise allocation for each menu element, and, as we have discussed, this requires an interpretation such as a product distribution for combinatorial valuations.
To test the flexibility of product distributions, we establish the first baseline as follows:

\begin{table}[t]
    \caption{Effect of the support size of the initial distribution ($D$) in \name~on CATS across different environments. Revenue increases dramatically when $D$ increases from 1 to 2. \label{tab:D}}
    \centering
    \begin{tabular}{ccccccc}
        \toprule
        \textbf{Environment} & \textbf{\# Items (m)} & $D=1$ & $D=2$ & $D=4$ & $D=8$ & $D=16$ \\
        \midrule
        \multirow{3}{*}{\makecell{CATS-Regions \\ \footnotesize Normal Private Valuations}} 
        & 50  & 278.82 & 589.50 & 596.67 & 603.70 & 595.14\\
        & 100 & 258.18 & 364.29 & 372.49 & 389.51 & 388.06 \\
        & 150 & 291.69 & 338.52 & 368.00 & 394.28 & 383.24 \\
        \midrule
        \multirow{3}{*}{\makecell{CATS-Arbitrary \\ \footnotesize Uniform Private Valuations}}
        & 50  & 287.98 & 557.06 & 563.70 & 560.71 & 561.51\\
        & 100 & 279.75 & 425.94 & 426.80 & 434.77 & 428.53  \\
        & 150 & 318.97 & 383.44 & 396.71 & 420.75 & 411.86\\
        \bottomrule
    \end{tabular}
\end{table}
%
\begin{table} [t]
    \caption{The Effect of increasing $D$ (the support size of initial distributions) under varying menu sizes $K$ (the number of elements in a menu). The default value of $K$ is 5000 when $m\le100$, and 20,000 otherwise.
    \label{tab:DJ} }
    \centering
    \begin{tabular}{CRCRCRCRCRCRCRCRCRCRCR}
        \toprule
        % \multicolumn{2}{c}{\multirow{2}{*}{}} &
        % \multicolumn{2}{l}{\multirow{2}{*}{Alg.}} &
        % \multicolumn{10}{c}{Setting}\\
        

        \multicolumn{4}{c}{Menu Size} &
        \multicolumn{4}{c}{$K/4$} & 
        \multicolumn{4}{c}{$K/2$} &
        \multicolumn{4}{c}{$K$} & 
        \multicolumn{4}{c}{$K*2$}\\

        \cmidrule(lr){1-4}
        \cmidrule(lr){5-8}
        \cmidrule(lr){9-12}
        \cmidrule(lr){13-16}
        \cmidrule(lr){17-20}
        \multicolumn{2}{c}{\textbf{Environments}} &
        \multicolumn{2}{l}{$m$} &
        \multicolumn{2}{c}{$D$=1} & 
        \multicolumn{2}{c}{$D$=2} &
        \multicolumn{2}{c}{$D$=1} & 
        \multicolumn{2}{c}{$D$=2} &
        \multicolumn{2}{c}{$D$=1} & 
        \multicolumn{2}{c}{$D$=2} &
        \multicolumn{2}{c}{$D$=1} & 
        \multicolumn{2}{c}{$D$=2} \\

        \cmidrule(lr){1-4}
        \cmidrule(lr){5-6}
        \cmidrule(lr){7-8}
        \cmidrule(lr){9-10}
        \cmidrule(lr){11-12}
        \cmidrule(lr){13-14}
        \cmidrule(lr){15-16}
        \cmidrule(lr){17-18}
        \cmidrule(lr){19-20}
        
        \multicolumn{2}{c}{\multirow{3}{*}{\makecell{CATS-Regions \\ \footnotesize Normal Private Valuations}}} & 
                               \multicolumn{2}{l}{50}  & \multicolumn{2}{l}{228.34} & \multicolumn{2}{l}{575.52} & \multicolumn{2}{l}{259.95} & \multicolumn{2}{l}{568.94} & \multicolumn{2}{l}{278.82} & \multicolumn{2}{l}{589.50} & \multicolumn{2}{l}{315.88}  & \multicolumn{2}{l}{602.98}\\
        \multicolumn{2}{c}{} & \multicolumn{2}{l}{100} & \multicolumn{2}{l}{213.26} & \multicolumn{2}{l}{324.04} & \multicolumn{2}{l}{226.11} & \multicolumn{2}{l}{345.51} & \multicolumn{2}{l}{258.18} & \multicolumn{2}{l}{364.29} & \multicolumn{2}{l}{270.65}  & \multicolumn{2}{l}{419.12}\\
        \multicolumn{2}{c}{} & \multicolumn{2}{l}{150} & \multicolumn{2}{l}{245.22} & \multicolumn{2}{l}{312.82} & \multicolumn{2}{l}{268.78} & \multicolumn{2}{l}{318.21} & \multicolumn{2}{l}{291.69} & \multicolumn{2}{l}{338.52} & \multicolumn{2}{l}{302.04}  & \multicolumn{2}{l}{385.08}\\
        
        \cmidrule(lr){1-4}
        \cmidrule(lr){5-6}
        \cmidrule(lr){7-8}
        \cmidrule(lr){9-10}
        \cmidrule(lr){11-12}
        \cmidrule(lr){13-14}
        \cmidrule(lr){15-16}
        \cmidrule(lr){17-18}
        \cmidrule(lr){19-20}
        
        \multicolumn{2}{c}{\multirow{3}{*}{\makecell{CATS-Arbitrary \\ \footnotesize Uniform Private Valuations}}} & 
                               \multicolumn{2}{l}{50}  & \multicolumn{2}{l}{238.96} & \multicolumn{2}{l}{546.50} & \multicolumn{2}{l}{261.61} & \multicolumn{2}{l}{551.78} & \multicolumn{2}{l}{287.98} & \multicolumn{2}{l}{557.06} & \multicolumn{2}{l}{303.53}  & \multicolumn{2}{l}{561.28}\\
        \multicolumn{2}{c}{} & \multicolumn{2}{l}{100} & \multicolumn{2}{l}{230.84} & \multicolumn{2}{l}{357.99} & \multicolumn{2}{l}{254.20} & \multicolumn{2}{l}{408.45} & \multicolumn{2}{l}{279.75} & \multicolumn{2}{l}{425.94} & \multicolumn{2}{l}{305.11}  & \multicolumn{2}{l}{438.27}\\
        \multicolumn{2}{c}{} & \multicolumn{2}{l}{150} & \multicolumn{2}{l}{297.22} & \multicolumn{2}{l}{355.07} & \multicolumn{2}{l}{303.08} & \multicolumn{2}{l}{361.01} & \multicolumn{2}{l}{318.97} & \multicolumn{2}{l}{383.44} & \multicolumn{2}{l}{343.19}  & \multicolumn{2}{l}{404.30}\\
        \bottomrule
    \end{tabular}
\end{table}

(1) \textbf{\bundle}: An adaption of RochetNet, interpreting its item-wise allocations as product distributions. Calculating bidder values remains intractable due to the need to enumerate all bundles. We address this by employing the \emph{Gumbel-SoftMax} technique~\cite{jang2017categorical}, which enables sampling from product distributions and backpropagation through the samples to update item-wise allocations. During training and testing, we use these samples to estimate bidder values. Empirically, item-wise allocations usually converge to binary vectors (0s or 1s) after training. In such scenarios, estimations of bidder values at test time are accurate, thereby ensuring that the mechanism is DSIC. If convergence to 0/1 vectors does not occur, DSIC is not exactly achieved in this baseline.

% making the calculation of bidder values tractable and ensuring DSIC. \dcp{rather than rest of sentence can we explain what we do at test time when this is not the case?} \tw{If that’s not the case, we estimate by sampling. Although we observed only binary vectors for the checkpoints we examined, we cannot guarantee DSIC. But it seems that better solutions are unlikely because enumeration is indeed intractable in scenarios with 100+ items. Should we emphasize that these results might be non-DSIC?} \dcp{I think 1-2 sentences saying what we do, and noting it can make it non-DSIC}.


To better understand the performance of \name~and \bundle, we also fix the allocations in RochetNet menus and only learn the prices using the same gradient-based optimization method as in RochetNet. Specifically, we have the following additional baselines:

(2) \textbf{\bigbundle}: This baseline focuses on large bundles, including the grand bundle (that includes all items) and those nearest in size to the grand bundle. When the menu size prevents the inclusion of all bundles of a certain size, selection is random, %(or can be pre-defined, in principle), 
favoring bundles with higher item counts. For instance, with 3 items and a menu size of 3, the menu would include $[1,1,1]$ (the grand bundle) and a random subset of bundles containing $2$ items, such as $[1,1,0]$ and $[0,1,1]$.

(3) \textbf{\smallbundle}: Similar to \bigbundle, but it prioritizes minimal item allocation, along with the grand bundle; i.e., it begins with single-item bundles and expands as the menu size permits.

(4) \textbf{\grandbundle}: A simple baseline that sets a single price for the grand bundle. The price is determined through a grid search based on maximum training set revenue;  performance, as with all methods, is reported on the test set.
%
\begin{table}[t]
    \caption{Revenue comparison against baselines across different CATS environments. The number of items is fixed at $m=50$, and we increase the valuation function size: $a = 10, 20, 30, 40$, and $50$ as maximum XOR atoms per valuation, corresponding to the {\em maxbid} parameter in CATS. \label{tab:exp_results_xor}}
    \centering
    \begin{tabular}{ccccccc}
        \toprule
        \textbf{Environment} & \textbf{Baseline} & $a=10$ & $a=20$ & $a=30$ & $a=40$ & $a=50$ \\
        \midrule
        \multirow{5}{*}{\makecell{CATS-Regions \\ \footnotesize Uniform Private Valuations}} 
        & \grandbundle & 314.46 & 309.11 & 316.04 & 320.61 & 314.35 \\
        & \bigbundle & 374.28 & 369.29 & 357.91 & 372.39 & 363.13 \\
        & \smallbundle & 328.95 & 328.92 & 323.44 & 333.00 & 326.58 \\
        & \bundle & 308.81 & 313.24 & 317.14 & 318.15 & 310.60 \\
        & \name & \textbf{533.42} & \textbf{528.46} & \textbf{528.26} & \textbf{539.92} & \textbf{537.36} \\
        \midrule
        \multirow{5}{*}{\makecell{CATS-Regions \\ \footnotesize Normal Private Valuations}} 
        & \grandbundle & 322.74 & 301.54 & 310.38 & 304.38 & 334.95 \\
        & \bigbundle & 434.32 & 375.51 & 404.74 & 381.05 & 430.24 \\
        & \smallbundle & 326.98 & 307.81 & 332.39 & 313.76 & 342.23 \\
        & \bundle & 301.47 & 297.34 & 317.10 & 302.04 & 327.32 \\
        & \name & \textbf{564.13} & \textbf{524.24} & \textbf{535.35} & \textbf{525.68} & \textbf{566.51} \\
        \midrule
        \multirow{5}{*}{\makecell{CATS-Arbitrary \\ \footnotesize Uniform Private Valuations}} 
        & \grandbundle & 331.21 & 334.43 & 330.33 & 351.01 & 336.68 \\
        & \bigbundle & 355.92 & 351.02 & 341.76 & 347.26 & 348.92 \\
        & \smallbundle & 352.34 & 354.58 & 346.36 & 354.87  & 353.58 \\
        & \bundle & 329.61 & 345.06 & 338.44 & 344.76 & 350.75 \\
        & \name & \textbf{565.54} & \textbf{583.60} & \textbf{568.01} & \textbf{579.01} & \textbf{581.39} \\
        \midrule
        \multirow{5}{*}{\makecell{CATS-Arbitrary \\ \footnotesize Normal Private Valuations}} 
        & \grandbundle & 381.51 & 335.44 & 323.52 & 320.28 & 358.83 \\
        & \bigbundle & 470.63 & 349.70 & 346.39 & 340.59 & 381.13 \\
        & \smallbundle & 402.23 & 341.79 & 337.44 & 332.90 & 368.26 \\
        & \bundle & 367.44 & 329.28 & 333.88 & 327.57 & 365.40 \\
        & \name & \textbf{664.94} & \textbf{564.90} & \textbf{552.77} & \textbf{548.22} & \textbf{615.93} \\
        \bottomrule
    \end{tabular}
\end{table}

\subsection{Setup}


We did not extensively fine-tune the flow model architecture, as the initial trial already yielded satisfactory results. This suggests that our formulation of the ODE is well-suited to the needs of the CA settings, making the optimization of the flow model relatively straightforward.

For the \name\ model, the $Q$ network comprises three 128-dimensional tanh-activated fully connected layers. When $m>100$, we increase the width of the last layer to 256. The $\sigma$ network is simpler and has two 128-dimensional tanh-activated fully connected layers. We did not extensively fine-tune this architecture, as the initial trial already yielded satisfactory results. This suggests that our formulation of the ODE, including its functional form (Eq.~\ref{equ:varphi}) and initial conditions (Eq.~\ref{equ:init_dist}), is well-suited to CA settings, allowing flexible choices of model architectures.
%\dcp{comment, e.g. footnote: did we need a lot of hyperparameter tuning?}

Two important hyper-parameters are $D$, the support size of the initial distribution, and $K$, the menu size. By default, $D$ is set to 8, a relatively small number. $K$ is 5000 when $m\le 100$ and is 20000 otherwise. This menu size setting is the same for both our method, \smallbundle, \bigbundle, and \bundle.
% \dcp{point later to where this is discussed?}
Notably, the selected menu sizes are adequate to encompass all possible bundles for smaller numbers of items, such as $m=5$ or $10$. We will show the impact of different values of $D$ and $K$ in ablation studies. 

Our menu optimization is conducted using the Adam optimizer with a learning rate of 0.3. $\lambda_{\textsc{SoftMax}}$ is increased from 0.001 to 0.2 over the course of training. For comprehensive details on our hyper-parameter settings, please refer to the codebase  provided with our submission. For the baselines, we fine-tuned their hyper-parameters so that they perform significantly better than the default RochetNet setting. The modifications are obtained by \jf{performing a gridsearch to obtain the optimum $\lambda_{\textsc{SoftMax}}$ and learning rate that yields the best revenue and also guarantees convergence. Both \smallbundle and \bigbundle uses learning rate of $0.3$ and $\lambda_{\textsc{SoftMax}}$ of 2, while \bundle uses learning rate of $0.05$ and $\lambda_{\textsc{SoftMax}}$ of 20.}

% We also fine-tune   and  For example, we gradually decrease the learning rate from $1e\shortn 2$ to $1e\shortn 4$ for training stability.
% \dcp{note will be available in future?}


\subsection{Results}

% \begin{table}[t]
%     \centering
%     \caption{
%     \label{tab:menu_support}}
%     \begin{tabular}{lccccccc}
%         \toprule
%         Menu Support Size & 1 & 2 & 4 & 8 & 32 & 128 \\
%         \midrule
%         CATS-Regions, normal, m=10 & 176.13, 176.10 & 174.13, 173.85 & 174.28 & 173.96\\
%         CATS-Regions, normal, m=50 & 278.56, 278.82 & 589.50 &  \\
%         CATS-Regions, normal, m=100 & 258.18 & 364.29, 353.71 & \\
%         CATS-Regions, normal, m=150 & 291.69 & 338.52\\
%         CATS-Arbitrary, m=10 & \\
%         CATS-Arbitrary, uniform, m=50 & 287.98 & 557.06\\
%         CATS-Arbitrary, uniform, m=100 & 279.75 & 425.94 \\
%         CATS-Arbitrary, uniform, m=150 & 318.97,316.84 & 383.44\\
%         \bottomrule
%     \end{tabular}
% \end{table}

\begin{figure}
    \centering
    \includegraphics[width=\linewidth]{figures/lc_a.pdf}
    \caption{Learning curves of \name~and baselines on \texttt{CATS Regions} with uniform valuation distributions with different valuation function sizes. The two rows are results for $a=10$ and $50$ XOR atoms per valuation, respectively. The three columns shows the changes of test revenue as a function of the number of training iterations, wall time in seconds, and the number of training samples, respectively.
    \label{fig:lca}}
\end{figure}

\textbf{Revenue on CATS and SATS}. Table~\ref{tab:exp_results} shows the revenue of our method compared against baselines. Our method performs consistently and significantly better when the number of items is large ($m>10$), achieving revenues gains of 1.2-3.6$\times$. The learning curves in Fig.~\ref{fig:lcm} further illustrate this advantage. The best performing baseline consistently requires 3000 seconds to converge, whereas \name~converges within approximately 140-180 seconds when $m=50$ and $100$, and within 2200 seconds when $m=150$. This translates to a 1.3-21.4$\times$ improvement in training speed.

When the number of items is small ($m=5$ and $10$), baselines with a menu size of 5000 can effectively cover all possible bundles. Similarly, in the SATS environment, where the number of possible bundles is $2400$, a menu size of $5000$ is sufficient. Although these settings are not the primary focus of our method, \name~can still achieve higher or comparable revenue relative to the baselines, as shown in the first two columns of Table~\ref{tab:exp_results} and Table~\ref{tab:sats}.

Among the baselines, \grandbundle~has relative better performance on CATS. Moreover, fixed allocation strategies (\smallbundle~and \bigbundle) outperform the full-fledged \bundle. A possible reason is that menu sizes of 5K or 20K remain negligible compared to the vast number of possible bundles like $2^{50}$ or $2^{150}$, but can pose a challenge for deep learning optimization. Therefore, the potential benefit of increased flexibility are over-weighed by the difficulty in optimization. This highlights an advantage of our method: while allowing better flexibility, it formulates an optimization problem that is more tractable, thereby enabling significantly improved performance.

\textbf{The support size of bundle distributions}. Table~\ref{tab:D} provides insights into why our method has superior performance. When we reduce the support size of initial distributions ($D$) to 1, each menu element deterministically assigns a single bundle to the bidder. This eliminates a key advantage of our method as it can no longer represent a distribution over bundles. Correspondingly, we observe a dramatic drop in revenue when $D$ is decreased from 2 to 1. For example, in the CATS \texttt{Regions} environment with normal distributions and 50 items, revenue declines sharply from 589.50 to 278.82. This trend remains consistent when we vary the menu size, as shown in Table~\ref{tab:DJ}. This pronounced performance gap between $D=1$ and $D=2$ highlights the importance of maintaining a randomized distribution over bundles in differentiable economics in CA settings---a capability uniquely enabled by our method.
%
Despite this loss of expressiveness when $D=1$, we find that our method can still outperform \bundle. This is because, even when optimizing a deterministic bundle for each menu element, we are ``searching" directly within the bundle space and, in principle, can reach any possible bundle. By contrast, as we have discussed, product distributions can represent only a limited subset of possible bundles. Therefore, our method retains greater flexibility than product distributions even when $D=1$.

\textbf{Menu size and Valuation function size}. Table~\ref{tab:DJ} presents the performance of our method under varying menu sizes ($K$), specifically when they are halved or quartered, and when they are doubled. As discussed, a randomized distribution over bundles is crucial in each of these settings, as revenue drops sharply when $D$ decreases to 1. Furthermore, increasing the menu size tends to improve performance, although the gains are modest when the item count is relatively low. For example, in \texttt{CATS Regions} with normal distributions, when $m=100$, increasing the menu size from $K/4$ to $K*2$ leads to a $29.34\%$ performance boost (rising from 324.04 to 419.12), in contrast to a merely $4.77\%$ enhancement when $m=50$ (rising from 575.52 to 602.98). Increasing the maximum number of XOR atoms per valuation from $10$ to $50$ has minimal effects on the performance of both our method and the baselines, as evidenced in Table~\ref{tab:exp_results_xor} and Fig.~\ref{fig:lca}.

% Results are reported for four \dcpadd{environments}: CATS-Regions with Uniform Private Valuations and  Normal Private Valuations, CATS-Arbitrary with Uniform Private Valuations and  Normal Private Valuations. with varying XOR \dcpadd{valuation function} sizes.

% To investigate the impact of menu support size on \name's performance, we evaluate revenue across different menu sizes in the network architecture.  \dcp{menu size, not $D$ for distribution support?  if yes, then `support` prob not a good word} Table~\ref{tab:menu_support} presents the results for menu sizes ranging from 2 to 128, using the Uniform Private Valuations model in CATS-Regions, with number of items of 50.
%550.89 & 555.05 & 552.79 & 553.67

% \begin{table}[t]
%     \centering
%     \caption{ The Effect of increasing $D$ ()
%     \label{tab:menu_support}}
%     \begin{tabular}{lccccccc}
%         \toprule
%         Menu Support Size & 1 & 2 & 4 & 8 & 32 & 128 \\
%         \midrule
%         CATS-Regions, normal, m=10 & 176.13, 176.10 & 174.13, 173.85 & 174.28 & 173.96\\
%         CATS-Regions, normal, m=50  & 315.88 & 602.98 &  \\
%         CATS-Regions, normal, m=100 & 270.65 & 419.12 & \\
%         CATS-Regions, normal, m=150 & 302.04 & 385.08\\
%         CATS-Arbitrary, m=10 & \\
%         CATS-Arbitrary, uniform, m=50  & 303.53 & 561.28\\
%         CATS-Arbitrary, uniform, m=100 & 305.11 & 438.27 \\
%         CATS-Arbitrary, uniform, m=150 & 343.19 & 404.30\\
%         \bottomrule
%     \end{tabular}
% \end{table}

%
% \begin{enumerate}
% \item 
% In particular we adopt a bundle-variation on {\em RochetNet}, which we call \dcp{BundleRochetNet?} 
%
%This parameterizes a menu of \dcpadd{item-wise allocation probabilities} and their associated payments, updating them using gradient descent to minimize negated expected revenue~\cite{dutting2024optimal}. 
%
% For this, we replace the softmax function of traditional RochetNet~\cite{dutting2024optimal}
% with a {\em Gumbel-softmax}, ensuring differentiability in this setting. \dcp{need more here---explain how it in effect rounds to get a single 0/1 bundle per menu element}.
% In this way, BundleRochetNet \dcp{?}
% has a representation
% that \dcpadd{is moderately 
% expressive, limited by deterministic menu elements and the size of the menu.}

% \end{enumerate}

% A more expressive class of baselines involves offering the buyer a menu of choices. While this approach remains tractable by limiting the menu size, it accommodates a \dcpadd{more flexible allocation and payment rule}. 
%dcp cut and in principle capable of recovering other menu-based baselines  such as AMA-based approaches with a limited .
%

% Despite its potential, we find that BundleRochetNet \dcp{?}
% struggles with scalability. Gradient-based updates become unstable and suboptimal when searching for a few thousand menu items in an exponentially-large bundle space. In fact, 
% baseline.
% Results are reported for four \dcpadd{environments:} CATS-Regions with Uniform Private Valuations and  Normal Private Valuations, CATS-Arbitrary with Uniform Private Valuations and  Normal Private Valuations.
